A Testbed for Transiently Powered Computers

Transiently Powered Computers (TPCs) are novel devices that are battery-less and operate using only ambient energy. Therefore TPCs are prone to frequent power interruptions, and such the need for developing TPC-centric algorithms is a necessity. We advocate that only through a common experimental environment, accessible to everyone, a proper comparison of newly developed algorithms for TPCs can be realized. Moreover, only through access to various TPC testbeds---distributed geographically throughout the world---a proper applications testing and validation are possible. We enlist properties and features that any TPC testbed should have, calling for more coordinated action in this domain of TPC research. Finally, we present (to the best of our knowledge) world's first Internet-accessible testbed for TPCs.

==> arch.tex <==
	
% \usepackage{tikz} % needed4: tikz pics
\tikzstyle{a} = [rectangle, draw=black!90, node distance=8mm, fill=white!20, text width=12mm, text centered, rounded corners, minimum height=2em, thick]
\tikzstyle{l} = [draw=black!90, -,very thick]
\tikzstyle{sl} = [draw=black!90, -,thick]
\tikzstyle{A} = [ shape=ellipse, minimum size=0.5cm,  text=black, thick, draw=black!90, align=center]
\tikzstyle{WISP} = [scale=0.5,shape=rectangle,minimum size=5mm,  text=white,fill=black!90];
\tikzstyle{TAG} = [scale=0.6,shape=rectangle,minimum size=3mm,  text=white,fill=black!90];
\tikzstyle{sTAG} = [scale=0.4,shape=rectangle,minimum size=4mm,  text=white,fill=black!90];

\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{shadows,shapes,arrows}





\begin{tikzpicture}
\newsavebox{\tagSquare}
\savebox{\tagSquare}{ \node (Wm) at (0,0) {};
	\draw[l] (-3.2mm,3mm) --(3mm,3mm)--(3mm,-3mm)--(-3mm,-3mm)--(-3mm,3mm);
	\draw[l](-3mm,3mm)--(3mm,-3mm);
	\draw[l](-3mm,-3mm)--(3mm,3mm);
	\node [TAG](Wm) at (0,0) {t};}
	
\newsavebox{\tagLong}
\savebox{\tagLong}{
	\node [](Wm) at (0,0) {};\node [sTAG] at (-5mm,0mm) {};
	\node [sTAG] at (5mm,0mm) {};
	\draw[sl] (-4.5mm,0.5mm) --(-3mm,0.5mm)--(-3mm,-0.5mm)--(-2mm,-0.5mm)--(-2mm,0.5mm)--(-1mm,0.5mm)--(-1mm,-0.5mm)--(-0mm,-0.5mm)--(-0mm,0.5mm)--(1mm,0.5mm)--(1mm,-0.5mm)--(2mm,-0.5mm)--(2mm,0.5mm)--(3mm,0.5mm)--(3mm,-0.5mm)--(4.5mm,-0.5mm);};

\newsavebox{\WISP}
\savebox{\WISP}{
	\node [WISP](Wm) at (-0,0) {w};
	\draw[l] ([xshift=-10mm,yshift=0mm]Wm.north) --([xshift=10mm,yshift=0mm]Wm.north);};

\newsavebox{\wave}
\savebox{\wave}{
	\draw [-] (10mm,8mm)  arc (60:120:20mm) node {};
	\draw [-] (5mm,6mm)  arc (60:120:10mm) node {};}

\draw[use as bounding box,transparent] 
		(-45mm,-6mm) rectangle (50mm,70mm);
			
\node (z) at (0,-1mm) {};
\node [a](host) at (z) {Host};
\node [a](c) at ([xshift=-30mm,yshift=0mm]z) {Client};
\node [a](r) at ([xshift=0mm,yshift=18mm]z) {Reader};
\node [](A1) at ([xshift=-25mm,yshift=0mm]r) {};
\node [](A2) at ([xshift=25mm,yshift=0mm]r) {};
\node [A](Ant1) at (A1) {Antenna1};
\node at (A1) {\usebox{\wave}};
\node [A](Ant2) at (A2) {Antenna2};
\node at (A2) {\usebox{\wave}};

%connections
\draw[-] (r) --(Ant2) ;
\draw[-] (r) --(Ant1);
\draw[-] (r) --(host)node[midway,above,sloped] {\scriptsize{LLRP}};
\draw[-] (c) --(host)node[midway,above,sloped] {\scriptsize{SSH}};



%single WISP
\node [rotate = 30] at (-25mm,46mm) {\usebox{\WISP}};
\draw[-latex] (-14mm,48mm) arc (0:30:12mm) node[right] {$\; \; \theta$};

%axis
\node [] at (-40mm,48mm) {
	\begin{tikzpicture}
		%axis
		\draw (0,0) -- (0,60mm);
		%ticks
		\foreach \y in {10,20,...,50}
		    \draw (0.5mm,\y mm) -- (-2mm,\y mm) 
		     node[anchor=east] {\y}; 
	\end{tikzpicture}
};
\draw[dashed,thick] (-5mm,23mm) -- (-5mm,70mm);

% TAG cloud:
\node [] at (25mm,50mm) {
	\begin{tikzpicture}
	%WISP
	\node [] at (25mm,40mm) {\usebox{\WISP}};
	
	%WISP
	\node [] at (25mm,50mm) {\usebox{\WISP}};
	\node [rotate=5] at (25mm,60mm) {\usebox{\WISP}};
	\node [rotate=5] at (40mm,45mm) {\usebox{\WISP}};
	\node [rotate=-5] at (10mm,55mm) {\usebox{\WISP}};
	
	%squareTag
	\node [](Wm) at (14mm,35mm) {\usebox{\tagSquare}};
	\node [](Wm) at (34mm,57mm) {\usebox{\tagSquare}};
	
	%longTag
	\node [rotate = 30] at (33mm,32mm) {\usebox{\tagLong}};
	\node [rotate = -20] at (8mm,47mm) {\usebox{\tagLong}};
	\node [rotate = 110] at (44mm,57mm) {\usebox{\tagLong}};
	\end{tikzpicture}
};

 
\end{tikzpicture}
